Neural Networks Enhancement with Logical Knowledge

In the recent past, there has been a growing interest in Neural-Symbolic Integration frameworks, i.e., hybrid systems that integrate connectionist and symbolic approaches to obtain the best of both worlds. In a previous work, we proposed KENN (Knowledge Enhanced Neural Networks), a Neural-Symbolic architecture that injects prior logical knowledge into a neural network by adding a new final layer which modifies the initial predictions accordingly to the knowledge. Among the advantages of this strategy, there is the inclusion of clause weights, learnable parameters that represent the strength of the clauses, meaning that the model can learn the impact of each clause on the final predictions. As a special case, if the training data contradicts a constraint, KENN learns to ignore it, making the system robust to the presence of wrong knowledge. In this paper, we propose an extension of KENN for relational data. To evaluate this new extension, we tested it with different learning configurations on Citeseer, a standard dataset for Collective Classification. The results show that KENN is capable of increasing the performances of the underlying neural network even in the presence relational data, outperforming other two notable methods that combine learning with logic.

==> SRL.tex <==
\chapter{KENN for Statistical Relational Learning}\label{ch:srl}

% \newcommand{\ad}[1]{{\color{blue}#1}}

\begin{TODO LIST}{TODO}
    \item Espandere descrizione:
    \begin{itemize}
        \item Far capire perche la prima versione di \kenn \ non puo essere usata coi dati relazionali (facendo riferimento anche al nuovo capitolo sull'implementazione)
        \item Concantrarsi sul l caso con regole n-arie, e specificare in seguito che nella partica si arriva di solito a arieta 2 o 3 e che ho testato solo con 2 (esempio e immagine con arieta' 2 per semplicita di esposizione)
        \item Usare l'esempio pratico dei documenti (per tutto il capitolo fare riferimento a tale esempio, mostrando come a partire dalle previsioni iniziali e dalle regole logiche si arrivi alle predizioni finali)
        \item Far capire come i vettori di indici sono passati
        \item mettere in chiaro che gli indici possono essere passati dell'utente finale (per esempio, in riferimento all'immagine della rappresentazione, non ci sono self loop nel grafo... questo solo perche il grafo da rappresentare non aveva self loops)
        \item Aggiunta dimostrazione formale del fatto che con mapping e reverse mapping i delta finali sono ancora la somma dei vari delta su tutti i grounding delle regole logiche (dimostrazione divisa in predicati binari e predicati unari) e di conseguenza si soddisfa la formula introdotta nel capitolo teorico su \kenn
        \item [opt] many sorted logic: aggiungendo una tabella per ogni dominio e usando piu volte la mapping function e la reverse su diverse tabelle e' possibile in teoria gestire diversi domini...\\
        In tal caso, per ogni termine di un predicato si definisce il dominio (come in PSL)
    \end{itemize}
\end{TODO LIST}

\begin{TODO LIST}{TODO}
    \item Aggiunta dettagli implementativi
    
\end{TODO LIST}

The first version of \kenn\ has been developed for multilabel classification. \AD{In this chapter we are interested in extending \kenn\ for relational data, where the single matrix representation introduced in Section~\ref{sec:architecture} can not be used.

More in details, in the single matrix representation the atomic formulas preactivations are stored as elements of a matrix $\bz$ with columns representing predicates and rows the individuals: element $z_{ij}$ contains the preactivation of $P_j(o_i)$, with $P_j$ the $j^{th}$ predicate and $o_i$ the $i^{th}$ object. 
% Such representation is exploited by \kenn\ to minimize the required computational effort: all the operations can be expressed as matrix operations, which are 
Such representation has an advantage: all the Knowledge Enhancer's internal calculations are implemented as matrix operations, which are particularly efficient when working with a GPU. However, the usage of $\bz$ is limiting since it is not possible to represent both unary and binary predicates in such matrix.
% and we would like for \kenn\ to consider also binary predicates, which is not possible with the matrix representation we have seen so far.

% \AD{
% Although the ideas behind \kenn\ could be applied to other types of tasks,the current implementation requires to represent data in a particular format. For this reason, it is not straightforward to use it in different contexts other than multi-label classification.
% }

% \TODO{
% Although the ideas behind \kenn\ could be applied to other types of tasks, the current implementation requires to represent data in a particular format, which is exploited by \kenn\ implementation to minimize the required computational effort. For this reason, \kenn\ can be applied for solving multi-label classification tasks, but it is not straightforward to use it in different contexts. }

% More in details, in the architecture introduced in Section~\ref{sec:architecture}, atomic formulas preactivations
% % to be modified
% are stored as elements of a matrix $\bz$.
% %  with columns representing predicates and rows the \TODO{groundings}. 
% \AD{Each column of $\bz$ refers to a unary predicate and each row refers to a specific object of the domain. All the atomic formulas in the row are obtained by substituting the free variable of a unary predicate (the one corresponding to the column) with that object.} Such representation is limiting and we would like for \kenn\
% % to be more flexible on the data structure used to store atomic formulas' values. We would like 
% to consider also binary predicates,\ which is not possible with the matrix representation we have seen so far.
% % \TODO{(spostare) each row of $\bz$ refers to a specific object of the domain and all the atomic formulas in the row are obtained by substituting the free variable of a unary predicate with that object.}

% We want to extend \kenn\ to work with graphs: instead of focusing only on unary predicates we need to use binary predicates as well. 
The next sections introduces the extension of \kenn\ for relational data, which can be applied on graphs.
%  mantaining the good time performances obtained by the usage of the single matrix representation. 
In designing this extension I paid particular attention to maintain the computational efficiency we have obtained in the previous version.}


%it would be preferable to keep the good time performances obtained by the usage of the single matrix representation. 


% \TODO{
% The idea is to develop a mapping function $m$ which can convert a custom representation into the matrix representation used so far. Moreover, we need a reverse mapping function $r$ which converts back the results to the required representation. In this way, we could keep the same implementation of KE.

% (reduce the graph problem to the original one...)




% % \begin{figure*}
% %     \makebox[\textwidth][c]{
% %         \includegraphics[scale=0.4]{imgs/m.jpg}
% %     }
% %     \caption{\kenn\ architecture: (a) for multilabel classification; (b) with structured NN output}
% %     \label{fig:mapping}
% % \end{figure*}


% In Fig.~\ref{fig:mapping}(a) it is shown the original version of \kenn: a neural network (NN) returns preactivations $\bz'$ based on features $\bx$, then \emph{Knowledge Enhancer} (KE) function takes $\bz'$ as input and returns $\delta \bz$, the update to be added to $\bz'$ in order to obtain the final preactivations $\bz$ (which in turn will be feed to the logistic function). Notice that the image is slightly different from the one of the original paper where the sum between $\bz'$ and $\delta \bz$ were performed inside KE together with the application of logistic regression. However, for the sake of this document, this representation is more useful.

% In Fig.~\ref{fig:mapping}(b) it is shown a new version of \kenn: here the results of the neural network have a different representation. Before applying KE, we use mapping function $m$ to store NN predictions into a matrix $M$ that can be processed by KE. A reverse mapping function $r$ is used to change the representation of KE outputs $\delta \M$ (changes to be applied to initial predictions) into the original representation and only then $\bz'$ and $\delta \bz$ are combined (notice that we require the addition to be defined for such a representation).


% }

\section{Relational data - Representation of a graph}

Before introducing the new version of \kenn\ we define the data structure we are going to use for representing the graph. Fig.~\ref{fig:representation} shows the data structures used to represent relational data. In the shown example there is a domain composed of three objects $O = \{o_0, o_1, o_2\}$, two unary predicates ($U_1$ and $U_2$) and one binary predicate ($B_1$). Fig.~\ref{fig:representation}(a) shows the graph representation with nodes and edges labelled with unary and binary predicates respectively. \AD{In this particular example the graph has no self-loops, meaning that $B_1(x,x)$ is not taken into account. Please notice that this constraint was added only for simplify the discussion of the example, and in general \kenn\ can work with self-loops.} 

Fig.~\ref{fig:representation}(b) shows the representation of the graph used by the new version of \kenn: it is composed of two matrices $\U$ and $\B$ for unary and binary predicates respectively and two vectors $s^x$ and $s^y$.
%  which give us information on the mapping from objects in $\U$ and couple of objects in $\B$.
% the substitutions applied on $\bar B_j$ on matrix $B$.

$\U$ is the same as $\bz$: it contains all the groundings of unary predicates (each column represents a predicate, each row a grounding), $\B$ contains the binary predicates (again, each column corresponds to a binary predicate, each row to a grounding of the two variables of the predicates). $s^x$ and $s^y$ contain the indexes of the pairs of objects in $\B$.
% (in respect to matrix $\U$) of objects that $\B$ is referring to.}
More precisely, if we consider a row $i$, $\B_{i,j}$ will correspond to the value of predicate $B_j$ for the substitution couple $(x | o_{s^x_i}, y | o_{s^y_i})$:
$$\B_{i,j} = B_j(o_{s^x_i},o_{s^y_i})$$

For instance, in Fig.~\ref{fig:representation}(b): $s^x_0 = 0$ and $s^y_0 = 1$, which means that row $0$ of matrix $\B$ is referring to the pair of objects $(o_0,o_1)$.

\begin{figure}[t]
	\centering
	\input{tikz/rel_representation}
    \caption{\TODO{Usare esempio pratico (papers e citazioni), mettere in chiaro che i valori riportati sono le preattivazioni (ottenute dalla rete base)}
        Relational data representation: in this example, three objects ($o_0$, $o_1$ and $o_2$), two unary predicates ($U_1$ and $U_2$) and only one binary predicate ($B_1$). (a): the graph representation; (b): the representation used by \kenn: matrix $\U$ contains all the groundings of unary predicates and matrix $\B$ the groundings of binary predicates. Vectors $s^x$ and $s^y$ contains the indexes of the objects $\B$ is referring to and they can be used to find a correspondence between values in $\B$ and values in $\U$. {\bfseries NB:} values refer to preactivations of the atomic formulas' truth values.}
    \label{fig:representation}
\end{figure}



\section{Unary and binary clauses}
\label{sec:SRL_representation}
We introduce a classification for clauses based on the number of variables they contains: a clause is unary if it contains only one free variable, binary if it contains two variables. For simplicity, in this thesis we don't take into account clauses with higher ariety. Notice however that this type of approach can be extended with \AD{predicates and} clauses with more than two variables.

Let $\clauses_U$ be the set of unary clauses and $\clauses_B$ the set of binary clauses. The Prior Knowledge is now defined as $\clauses = \clauses_U \cup \clauses_B$.

The idea now is to apply KE to the two sets separately.
% : the changes to be applied on binary predicates comes only from binary clauses, while the changes on unary clauses depends on both unary and binary clauses.
KE can be called directly on $\U$ using only the unary knowledge $\clauses_U$. This can be done since $\U$ contains only unary predicates and it represents the data in the same way of $\bz$ for the multi-label version of \kenn. The output of KE is a matrix that collects the changes to be applied to $\U$ based on unary clauses $\clauses_U$. We call it $\delta \U^u$ to distinguish it from $\delta \U^b$ (the changes to apply to matrix $\U$ based on binary clauses).

At this point we also need to increase the satisfaction of binary clauses. To do this we use the so called \emph{mapping function}, which maps the graph representation into a single matrix $\M$. Such matrix is used by the KE with $\clauses_B$. \AD{The KE returns $\delta \M$, a matrix of the same shape of $\M$ which contains the changes on the initial predictions induced by binary clauses. Finally, such matrix need to be converted in the original representation of the graph: the \emph{reverse mapping function} takes in input $\delta \M$ and outputs $\delta \U^b$ and $\delta \B$ which are added to $\U$ and $\B$ to obtain the final predictions.}

Fig.~\ref{fig:unary_binary} shows a high level overview of the entire model.

\begin{figure}[t]
	\centering
	\input{tikz/rel_overview}
    \caption{To obtain $\delta \U^u$, unary clauses $\clauses_U$ are used by KE directly on $\U$. The mapping function is used to find matrix $\M$. Then, the KE is applied to $\M$ using binary clauses $\clauses_B$. Finally, to obtain $\delta \U^b$ and $\delta \B$ the reverse mapping function is used.}
    \label{fig:unary_binary}
\end{figure}


% \TODO{The idea now is to apply KE to the two sets separately and use functions $m$ and $r$ only to manage $\clauses_B$.
% % Indeed, KE can already deal with unary clauses and we can apply KE to the values in $U$ using $\clauses_U$.
% In Fig.~\ref{fig:unary_binary} we see that a KE is called directly on $U'$ using only the unary knowledge $\clauses_U$. The result is called $\delta \U^u$ to distinguish it from $\delta \U^b$ (the changes to apply to matrix $U$ based on binary clauses).
% % , which is the set of unary clauses in our original Prior Knowledge $\clauses = \clauses_U \cup \clauses_B$.
% }

\section{Binary extensions of unary predicates}
\TODO{citare Neural Logic Machines (nel loro caso usano il verbo expand, ma di fatto fanno la stessa cosa... ma su tensori)}
Given a unary predicate $U_i$, we define its binary extensions as two binary predicates $U_i^x$ and $U_i^y$ such that:
$$
\forall x \ \forall y \ U_i^x(x,y) \leftrightarrow U_i(x)
$$
and
$$
\forall y \ \forall x \ U_i^y(x,y) \leftrightarrow U_i(y)
$$
Intuitively, the $U_i^x$ and $U_i^y$ are binary predicates that ignore one of the two inputs. For instance, let $Person(x)$ be the unary predicate that is true if $x$ is a person. The $Person^x(x,y)$ is the binary predicate corresponding to the sentence: ``The first object of the pair $(x,y)$ is a person''.

For each binary clause, we can substitute the original unary predicates with their binary extensions. For instance, the clause
$$c: \lnot U_1(x) \lor \lnot U_1(y) \lor B_1(x,y)$$
is converted to
$$c': \lnot U_1^x(x,y) \lor \lnot U_1^y(x,y) \lor B_1(x,y)$$

It is easy to prove that the truth value of $c'$ is the same of $c$:
$$\forall x \ \forall y \ \Big( U_i^x(x,y) \leftrightarrow U_i(x) \Big) \land \Big(U_i^y(x,y) \leftrightarrow U_i(y)\Big) \models c \leftrightarrow c'$$

Notice that while in $c$ there were both unary and binary predicates, in $c'$ all the predicates are binary. This is true for the original domain $O$, but they can be seen as unary predicates if we consider the domain of couple of objects ($O \times O$). Our new solution for relational data comes exactly from this new perspective: if we extend matrix $\B$ to contain also the new binary predicates $U_i^x$ and $U_i^y$, then we can apply directly the KE on the resulting matrix using $\clauses_B$.

In summary, binary clauses can be seen as unary clauses in the domain of pairs of objects. Since KE can deal with unary clauses, it can be used to enhance binary clauses as well.

Mapping function just need to return a matrix $\M$ which has a row for each pair of objects and a column for each binary predicate (including the binary extensions $U_i^x(x,y)$ and $U_i^y(x,y)$).



\section{Mapping function}
 The mapping function makes use of \emph{gather} function of TensorFlow which slices a given matrix according to an indices vector. In Fig.~\ref{fig:gather} an example of \emph{tf.gather} usage. For more details about \emph{tf.gather} see the official \href{https://www.tensorflow.org/api_docs/python/tf/gather}{TensorFlow documentation}.

\begin{figure}[t]
	\centering
	\input{tikz/gather_example}
    \caption{\emph{tf.gather} behaviour: given a matrix $\U$, it copies in a new matrix the rows of $\U$ based on the provided indices.}
    \label{fig:gather}
\end{figure}

Vectors $s^x$ and $s^y$ contain the indexes of the objects in $\U$ which are referred by matrix $\B$. For instance, in Fig.~\ref{fig:gather} $s^y_0=1$, which means that in the first row of $\B$ the $y$ variable of the binary predicates is substituted by object $o_1$ . Therefore, when \emph{tf.gather} is applied to $\U$ using $s^x$ ($s^y$) it generates a matrix containing the values of $U_i^x$ ($U_i^y$) corresponding to the grounding in $\B$. The mapping function just need to concatenate the resulting matrices with $\B$ to obtain the final matrix $\M$. Fig.~\ref{fig:mapping}~shows the implementation of mapping function.

The key point of this strategy is that we can apply the KE on matrix $\M$ using $\clauses_B$. The result $\delta \M$ is a matrix of the same shape of $\M$ which collects all the changes to be applied on atomic formulas due to binary clauses.

Now we just need to define the reverse mapping function, which copies $\delta \M$ values into the initial representation: it returns the final changes (generated from $\clauses_B$) that should be applied on unary ($\delta \U^b$) and binary ($\delta \B$) grounded predicates.

% to copy the unary predicates in the right spots of final matrix $\M$ (see \href{https://www.tensorflow.org/api_docs/python/tf/gather}{TensorFlow documentation} for a better description of \emph{tf.gather} function).

% In the shown example:
% $$
% s^x = \ensuremath{\begin{pmatrix}0\\0\\1\\1\\2\\2\end{pmatrix}}
% $$

% This is telling us that the first two rows of matrix $\B$
% % and of the final matrix $M$
% are referring to the object in row $0$ of $\U$, while the third and fourth row correspond to row $1$ in $\U$. By applying \emph{tf.gather} to matrix $\U$ and vector $s^x$ we generate a matrix which contains the unary predicates values for the objects referred by $s^x$. The same strategy is applied with $s^y$. Finally we concatenate the two resulting matrices with $\B$. The final matrix $\M$ can be seen as an extension of matrix $\B$ obtained by adding the missing binary predicates (the binary extensions of unary predicates). 



\begin{figure}[t]
	\centering
	\input{tikz/rel_mapping}
    \caption{\TODO{usare anche qui l'esempio, specificare almeno una regola logica e mettere dei valori sensati..., aggiungere altra immagine separate per l'applicazione del KE (sempre con lo stesso esempio) in cui si mostra esattamente cosa succede} The architecture of mapping function: it applies \emph{tf.gather} to $\U$ using as indices $s^x$ and $s^y$. The resulting matrices contain $\U$'s rows ordered as specified by the two vectors. Finally, using the concatenation it generates matrix $\M$ which can be provided as input to the KE together with the binary knowledge $\clauses_B$.}
    \label{fig:mapping}
\end{figure}



\section{Reverse mapping function}
\label{reverse}
From Fig.~\ref{fig:mapping} we can notice that we have multiple delta values for each grounded unary predicate inside matrix $\delta \M$. For instance, the values of $M_{0,2}$, $M_{2,0}$, $M_{3,0}$ and $M_{5,2}$ are all referring to $U_1(o_1)$ and they come from different grounding of the binary clauses.

The reverse mapping function works in reverse of the mapping function. The first step is to split $\delta \M$ in three matrices: $\delta \M^x$ contains the delta values for predicates of the form $U_i^x$, $\delta \M^y$ refers to predicates $U_i^y$ and $\delta \B$ to binary predicates $B_j$. 

% \AD{Notice that $\delta \M^x$ does not contain any predicates that refers to variable $y$ (the same is true for $\delta \M^y$ and variable $x$). Therefore, we can see the predicates referred by $\delta \M^x$ as the original unary predicates (instead of using their binary extensions). Indeed, $\delta \M^x$ has a similar structure as $\U$, with the exception that multiple rows refer to the same object.}

The proposed changes for binary predicates ($\delta \B$) are already usable. In other words, they can be directly added to matrix $\B$ to obtain final preactivations $\B'$: 
$$\B' = \B + \delta \B$$

For the unary predicates it is needed an additional step: we have to collect all the changes referring to the same atomic formula, sum them together and put the results in the right position of matrix $\delta \U^b$. This is achieved through the use of \emph{scatter\_nd} function of TensorFlow which works in reverse of \emph{tf.gather}. Indeed, while for \emph{tf.gather} the indices refer to the input matrix, with \emph{tf.scatter\_nd} they refer to the output matrix. Fig.~\ref{fig:scatter} shows an example of \emph{tf.scatter\_nd} usage (see \href{https://www.tensorflow.org/api_docs/python/tf/scatter_nd}{TensorFlow documentation} for more details). Notice that when the indices vector contains multiple indices with the same value, the corresponding rows are summed together before being copied. 

\begin{figure}[t]
	\centering
	\input{tikz/scatter_example}
    \caption{\emph{tf.scatter} behaviour: it copies the rows of a matrix in the specified indices. When multiple indices are equivalent it sums the corresponding rows.}
    \label{fig:scatter}
\end{figure}

Using \emph{tf.scatter\_nd} with indices vector $s^x$, \kenn\ can automatically sum up all the contributions of the same atomic formula found in $\delta \M^x$ and put the results in the right position inside a new matrix called $\delta \U^x$. The same strategy is applied for calculating $\delta \U^y$ matrix. Then the two matrices are summed together to obtain $\delta \U^b$:
$$\delta \U^b = \delta \U^x + \delta \U^y$$
Finally, the preactivations of unary predicates are calculated as:
$$\U' = \U + \delta \U^u + \delta \U^b$$

The detailed architecture of the reverse mapping function can be seen in Fig.~\ref{fig:reverse_mapping}.


\begin{figure}[t]
	\centering
	\input{tikz/rel_reverse_mapping}
    \caption{\TODO{Continuare anche qui con l'esempio solito} The architecture of the reverse mapping function: first, it splits $\delta \M$ into three matrices which contain the improvements to apply to predicates $U_i^x$, $U_i^y$ and $B_i$. It then makes use of \emph{tf.scatter\_nd} to add all the values referring to the same atomic formulas and store them in the right position in $\delta \U^x$ and $\delta \U^y$. Finally, the two matrices are added together to obtain $\delta \U^b$.}
    \label{fig:reverse_mapping}
\end{figure}


% \begin{figure*}
%     \makebox[\textwidth][c]{
%         \includegraphics[scale=0.09]{reverse_mapping.jpg}
%     }
%     \caption{The reverse mapping function projects the changes proposed by KE (with binary clauses $\clauses_B$) into the original data structure of the underlying graph. It makes use of \emph{tf.scatter\_nd} function, which works in reverse as \emph{tf.gather}: it sums up all the rows in $\delta \U^x$ that refer to the same object in $O$. In other words, it sums rows with the same value in $s^x$. The same is done for $\delta \U^y$ and $s^y$. The final matrices has the same shape as $U'$ and they are summed to it to obtain the final unary predictions $U$.}
%     \label{fig:reverse_mapping}
% \end{figure*}





{


% \begin{TODO LIST}{TODO}
%     \item Aggiungere spiegazione formale del perche' e' corretto (scatter\_nd calcola la somma su tutti i groundings...)
%     \item aggiungere in appendix descrizione di scatter\_nd e gather
% \end{TODO LIST}


}

==> acknowledgments.tex <==
\section*{Acknowledgments}
\DONE{I would like to thank Luciano Serafini, who supported and guide me during my Ph.D. Many thanks also to Alessandro Sperduti and Marco Gori for useful suggestions and feedbacks. I would also like to show my gratitude to Artur d'Avila Garcez who provide me with useful insights on my research during my period abroad at the Research Centre for Machine Learning of City, University of London. Finally, I thank Ivan Donadello for providing the knowledge base for VRD Dataset produced during his Ph.D. and for useful comments.}

==> collective_-_old.tex <==
\chapter{Experiments on relational data}\label{ch:collective}

\begin{TODO LIST}{TODO}
    \item Tests training ridotto
    \item Tests inductive
    \item Tests con LTN (anche qui, training ridotto, inductive, pochi hidden nodes)
    \item Altri dataset (ancora da decidere)...
    \item Far notare che non ho bisogno di applicare le regole logiche at inference time mentre SBR si (solo per inductive?)
    \item dire che con transductive anche kenn (che e satto pensato per inductive) e' come se applicasse le regole sulla loss (perche gli conviene settare i nodi sconosciuti usando le regole logiche)
\end{TODO LIST}

In this chapter we focus on experiments with relational data. More precisely, the relational version of \kenn\ was tested using three datasets for collective classification. In the task of collective classification we are interested in finding a classification for the nodes in a graph using both features of the nodes (the objects) and the information coming from the edges of the graph (relations between objects)~\citep{collective_classification}.

We focus on semi-supervised node classification, where labels are provided for a small subset of the graph and the model is trained using both labelled and unlaballed data. 

In a collective classification task there are two different learning paradigms: transductive and inductive learning. As in~\citep{GCN}, we focus on transductive learning where the goal is to provide predictions only of unlaballed data that is available at training time~\citep{zhu, yang}.

\section{Datasets}
As in \citep{GCN} and \citep{yang}, we use three citation network datasets: Citeseer, Cora and Pubmed~\citep{collective_classification}. In these datasets, the graph's nodes represent documents and the edges represent citations. The nodes' features are bag-of-words vectors, where an entry is zero if the corresponding word of the dictionary is absent in the document, and one if it is present. The classes to be predicted represent possible topics for a document.
Table~\ref{SRL_datasets} shows some figures of the three datasets. Label rate is the fraction of nodes used for training.

\begin{table}
    \caption{Datasets statistics}
    \centering
    \begin{tabular}{|l|l|l|l|l|l|}
        \hline
        Dataset & Features & Classes & Nodes & Edges & Label rate\\
        \hline
        \hline
        Cora & 1433 & 7 & 2708 & 5429 & 0.052\\
        \hline
        Citeseer & 3703 & 6 & 3327 & 4732 & 0.036\\
        \hline
        Pubmed & 500 & 3 & 19717 & 44338 & 0.003\\
        \hline
    \end{tabular}
    \label{SRL_datasets}
\end{table}

\section{The Prior Knowledge}
All the datasets taken in consideration are citation networks and the labels to be predicted are the documents topics. For this reason, the type of Knowledge used was the same for all the datasets.

\subsection{Simple Knowledge}
In a first experiment with logistic regression and Cora Dataset the knowledge was  composed of a single clause for each topic $T$:
$$
\forall x \ \forall y \ T(x) \land Cite(x,y) \to T(y)        
$$
which is telling \kenn\ that if a paper $x$ cite another paper $y$, then they should be about the same topic.

\subsection{Bibliography Knowledge}
\AD{Notice that the above axioms assume that one paper cites only papers of the same topic. In most of the cases this is not true. For instance, if the graph is fully connected the aximos are true only if all the papers are about the same topic. For this reason we propose a softer version that consider the topic of the bibliography as a whole.

The new type of knowledge, called Bibliography Knowledge, defines a new unary predicate $T_B$ for each topic $T$.} Intuitively, $T_B(x)$ should be true if the bibliography of paper $x$ can be classified as topic $T$.

For each topic, we define the clause:
$$
\forall x \ T_B(x) \to T(x)
$$
\noindent meaning that a paper must be classified with the same topic of its bibliography.

To calculate this bibliography predicates the model first multiplies the predictions of the base NN for the adjacency matrix of the citation graph and then it applies the softmax function to each row of the resulting matrix:
$$
\T^B = softmax(\A \T)
$$
\AD{
\noindent where $\T$ is the matrix containing the topics for each paper as predicted by the GCN (similar to the definition of $\bz$, each colum represents a topic and each row a node of the graph); $\A$ is the adjacency matrix of the citation graph: it contains all the citations between papers and is defined as the matrix with values $A_{ij} = Cite(o_i,o_j)$.
}

\section{Experimental setup}
In the first experiment on Cora dataset \AD{I used the Simple Knowledge and} I followed a similar strategy as previous experiments: \AD{the base NN was a logistic regression on top of which I added the Knowledge Enhancer. The logistic regression takes as input only the nodes features and it does not take into account relations. For this reason, by adding the knowledge, we could expect great improvements as compared to the base NN. Indeed, the relations are taken into account only on the level of the KE.}

In a second set of experiments on all the three datasets, Simple Knowledge was added to a Graph Convolutional Network (GCN)~\citep{GCN}\footnote{GCN are neural networks models which can be applied on graphs \citep{GCN}. The architecture is composed of multiple layers, each of which can be described by:
$$
H^{(l+1)} = \sigma\Big( \widetilde{D}^{-1/2} \widetilde{A} \widetilde{D}^{-1/2} H^{(l)} W^{(l)} \Big)
$$
where $H^{(l)}$ represents the output of layer $l$ (for the first layer $H^{(0)}$ is equal to the input features $X$), $\sigma$ is an activation function (typically a ReLU for the hidden layers), $\widetilde{A}$ is the adjacency matrix of the graph $A$ with the addition of self loops ($\widetilde{A} = A + I$) and $\widetilde{D}$ is the diagonal node degree matrix of $\widetilde{A}$: $\widetilde{D}_{i,i}= \sum_{j}{\widetilde{A}_{i,j}}$. Finally, $W^{(l)}$ is the weight matrix of layer $l$, which is trainable}. This is one of the best models for this type of tasks; moreover the authors provided the source code of the network making it easier to conduct experiments on it. The source code is available on \href{https://github.com/tkipf/gcn}{github} and it already provides all the code and data for testing with the three considered datasets. The experiments with GCN were conducted using the original hyper-parameters of~\citep{GCN}. The results obtained motivated a third set of experiments: I used again GCN as base NN, this time using Bibliography Knowledge.

Following \citep{GCN} and \citep{yang}, in all the experiments I used the same setup: the test set was composed of 1000 randomly selected nodes, while the training was splitted in two parts. The first one is a set containing labeled data created by randomly selecting 20 nodes per class; the second contains the remaining nodes as unlabeled data. Finally, all the evaluations were done on \kenn\ learned in an end-to-end fashion.

Notice also that the citations are known a priori (the edges of the graph are given as inputs). Therefore, when applying KE, it is possible to focus only on pairs of documents for which the $Cite(x,y)$ predicate is known to be true. Indeed, all the grounded clauses in the Prior Knowledge are automatically satisfied if $Cite(x,y)$ is false for the specific grounding. This means that clauses are always satisfied when the pair of documents do not cite one another and that KE would not apply any changes for such pairs of objects. For this reason, $s_i^x$, $s_i^y$ and $\B$ were generated using only pairs of object for which $Cite(x,y)$ is true reducing both train and test time. \AD{Moreover, $s_i^x$, $s_i^y$ and $\B$ can be directly calculated from the adjacency matrix provided in the GCN source code: the authors represented it as a sparse matrix which could be easily converted in the COO format (see \href{https://docs.scipy.org/doc/scipy/reference/generated/scipy.sparse.coo_matrix.html}{SciPy documentation} for more details). Indeed, the COO format is equivalent to the representation of graph data proposed in Section~\ref{sec:SRL_representation}.}


% \TODO{Moreover, finding the values of $s_i^x$, $s_i^y$ and $\B$ were particularly easy when using }

Finally, since each paper can not be classified with multiple classes, the activation used was the softmax function.


% Notice that the results obtained in Section~\ref{preact} were proved with the assumption that the activation is a logistic function. Therefore, there is not theoretic evidence that this approach can work. However, the results obtained give us empirical evidence that \kenn\ can work even with softmax activation.

% \TODO{Spostare in footnote:
% \section{Graph Convolutional Networks}
% Graph Convolutional Networks (GCN) are neural networks models proposed by Kipf and Welling in 2017 which can be applied on graphs \citep{GCN}. The architecture of GCN is composed of multiple layers, each of which can be described by:
% $$
% H^{(l+1)} = \sigma\Big( \widetilde{D}^{-1/2} \widetilde{A} \widetilde{D}^{-1/2} H^{(l)} W^{(l)} \Big)
% $$
% where $H^{(l)}$ represents the output of layer $l$ (for the first layer $H^{(0)}$ is equal to the input features $X$), $\sigma$ is an activation function (typically a ReLU for the hidden layers), $\widetilde{A}$ is the adjacency matrix of the graph $A$ with the addition of self loops ($\widetilde{A} = A + I$) and $\widetilde{D}$ is the diagonal node degree matrix of $\widetilde{A}$: $\widetilde{D}_{i,i}= \sum_{j}{\widetilde{A}_{i,j}}$. Finally, $W^{(l)}$ is the weight matrix of layer $l$, which is trainable.}

\section{Results}
\label{sec:results_collective}
Table~\ref{SRL_results} shows the results of \kenn\ on the three datasets using both LR and GCN: LR stands for Logistic Regression, \kenn$_{LR}$ and \kenn$_{GCN}$ correspond to \kenn\ applied on LR and GCN respectively. Finally, the superscripts $S$ and $B$ stands for Simple and Bibliography Knowledge.


\begin{table}[H]
    \caption{Results in terms of accuracy on the inductive variant of the task ordered by the amount of data used for training. The first three columns contains the results reported in~\citep{RNM}.}
    % , while my results are in the last three. Notice that the NN results are slightly different in the two versions}
    \centering
    \begin{tabular}{c|lll|lll}
        \% training & NN & SBR & RNM & NN & \kenn$_g$ & \kenn$_e$ \\
        \hline
        \rule{0pt}{3ex}\hspace{-0.12cm}
        10 & 0.645 & 0.650 & {\bfseries 0.685} & 0.591 & 0.603 & 0.591 \\
        &&  (+0.005) & {\bfseries (+0.040)} && (+0.012) & (-0.000) \footnote{The improvement in the case of \kenn$_e$ for 10\% of data was $-3.36 \cdot 10^-5$. This is approximated as zero in the table.}\\
        \rule{0pt}{3ex}\hspace{-0.12cm}
        25 & 0.674 & 0.682 & {\bfseries 0.709} & 0.644 & 0.661 & 0.659 \\
        &&  (+0.008) & {\bfseries (+0.035)} && (+0.017) & (+0.015)\\
        \rule{0pt}{3ex}\hspace{-0.12cm}
        50 & 0.707 & 0.712 & {\bfseries 0.726} & 0.685 & 0.691 & 0.701\\
        &&  (+0.005) & {\bfseries (+0.019)} && (+0.006) & (+0.016)\\
        \rule{0pt}{3ex}\hspace{-0.12cm}
        75 & 0.717 & 0.719 & 0.726 & 0.723 & 0.725 & {\bfseries 0.742} \\
        &&  (+0.002) & (+0.009) && (+0.002) & {\bfseries (+0.019)}\\
        \rule{0pt}{3ex}\hspace{-0.12cm}
        90 & 0.723 & 0.726 & 0.732 & 0.722 & 0.725 & {\bfseries 0.740} \\
        &&  (+0.003) & (+0.009) && (+0.003) & {\bfseries(+0.018)}\\
        \hline
        \hline
    \end{tabular}
    \label{inductive_results}
\end{table}



\begin{table}[H]
    \caption{Results in terms of accuracy on the transductive variant of the task ordered by the amount of data used for training. The first three columns contains the results reported in~\citep{RNM}.}
    % , while my results are in the last three. Notice that the NN results are slightly different in the two versions}
    \centering
    \begin{tabular}{c|lll|lll}
        \% training & NN & SBR & RNM & NN & \kenn$_g$ & \kenn$_e$ \\
        \hline
        \rule{0pt}{3ex}\hspace{-0.12cm}
        10 & 0.640 & 0.703 & {\bfseries 0.708} & 0.599 & 0.611 & 0.649 \\
        &&  (+0.063) & {\bfseries (+0.068)} && (+0.013) & (+0.050)\\
        \rule{0pt}{3ex}\hspace{-0.12cm}
        25 & 0.667 & 0.729 & {\bfseries 0.735} & 0.649 & 0.662 & 0.681 \\
        &&  (+0.062) & {\bfseries (+0.068)} && (+0.013) & (+0.032)\\
        \rule{0pt}{3ex}\hspace{-0.12cm}
        50 & 0.695 & 0.747 & {\bfseries 0.753} & 0.682 & 0.692 & 0.726\\
        &&  (+0.052) & {\bfseries (+0.058)} && (+0.010) & (+0.045)\\
        \rule{0pt}{3ex}\hspace{-0.12cm}
        75 & 0.708 & 0.764 & {\bfseries 0.766} & 0.705 & 0.709 & 0.755 \\
        &&  (+0.056) & {\bfseries (+0.058)} && (+0.004) & (+0.050)\\
        \rule{0pt}{3ex}\hspace{-0.12cm}
        90 & 0.726 & 0.780 & 0.780 & 0.728 & 0.747 & {\bfseries 0.785} \\
        &&  (+0.054) & (+0.054) && (+0.019) & {\bfseries(+0.057)}\\
        \hline
        \hline
    \end{tabular}
    \label{transductive_results}
\end{table}







\begin{table}[H]
    \caption{Results on the three citation networks datasets in terms of accuracy.}
    \centering
    \begin{tabular}{llll}
        & Cora & Citeseer & Pubmed \\
        \hline
        \rule{0pt}{3ex}\hspace{-0.12cm}
        ManiReg~\citep{ManiReg} &  59.5 & 60.1 & 70.7  \\
        LP~\citep{LP}    & 68   &  45.3 & 63.0 \\
        DeepWalk~\citep{deep_walk} & 67.2 & 43.2 & 65.3 \\
        Planetoid~\citep{planetoid} & 75.7 &  64.7 & 77.2 \\
        DCNN~\citep{DCNN} & 76.7 & 64.5 & 75.3 \\
        GAT~\citep{GAT}  & 83.2 &  71.0 & 78.0 \\
        GDEN~\citep{GDEN} & {\bfseries 85.1} & {\bfseries 72.8} & 78.9 \\
        \hline
        \rule{0pt}{3ex}\hspace{-0.12cm}
        LR  & 42.9 & - &  - \\
        \kenn$_{LR}^S$ & 77.4 & - & - \\
        \hline
        \rule{0pt}{3ex}\hspace{-0.12cm}
        GCN~\citep{GCN}  & 81.5 &  70.3 & {\bfseries 79.0} \\
        \kenn$_{GCN}^S$ & 77.8 & 63.8 & 75.4 \\
        \kenn$_{GCN}^B$ & 81.9 & 70.3 & 77.9 \\
        \hline
        \hline
    \end{tabular}
    \label{SRL_results}
\end{table}

In the first experiment using logistic regression \kenn\ confirmed to be capable of improving predictions of shallow networks. Moreover, the results are quite good considering the minimal effort required to obtain such results. Indeed, they were obtained just by adding few simple clauses into a simple network as LR and the accuracy obtained is outperformed only by the latest and more advanced methods. Moreover, in principle \kenn$_{LR}$ can work even in an inductive settings while other considered methods cannot. For instance, GCN and GDEN can be used only in the context of transductive learning, meaning that they cannot provide predictions for new nodes that were not provided during training~\citep{GCN, GDEN}. 

Notice that the results of \kenn$_{GCN}^S$ are not in line with the state of the art and more importantly there was a degradation on the predictions compared to the base NN (GCN).
% This behavior could appear counterintuitive since by setting clause weights to zero the model could ignore the clauses and returns directly the output of the GCN. 
These results could be explained by the fact that multiple groundings of the clauses could apply opposite changes on the same atomic formula. For instance, if a paper $x$ is cited by papers of two different topics, we have a contradiction since the effect of the knowledge is that $x$ should be classified with both topics. 
% Combined with the usage of softmax function as activation, this could be the reason of the poor performances of \kenn$_{GCN}^S$.

To obviate this problem, I created the Bibliography Knowledge and tested \kenn\ with GCN on it. As we can see from Table~\ref{SRL_results}, the results with this kind of knowledge are much better than the previous ones. However, there were no significant improvements over the base NN. A simple explanation could be that the capacity of GCN is big enough to make it easy for the model to represent solutions which satisfy our constraints. In other words, since the constraints are already satisfiable by GCN, the injected knowledge is redundant and it doesn't lead to improvements.

To test this hypothesis I made an additional experiment in which I tested the accuracy on Test Set with different numbers of GCN hidden nodes. Figure~\ref{fig:results_srl} shows the results.


The image confirmed the hypothesis: for all the three datasets \kenn\ produces an improvement over the base NN when the number of hidden nodes is low. Indeed, the two models' performances converge to the same value when increasing the number of hidden nodes. 
% \TODO{dire qui che cio potrebbe voler dire che se la rete base e' in grado di soddisfare i vincoli e si hanno molti dati kenn non va bene... in generale ha senso usare kenn su reti deep?? Booh.. altri esperimenti!}

Notice also that in the case of Citeseer \kenn\ have a more stable behavior than GCN.

\begin{figure}
    \makebox[\textwidth][c]{
        \includegraphics[scale=0.45]{Figures/results.png}
    }
    \caption{Results of \kenn\ and GCN in terms of accuracy with different values of hidden nodes}
    \label{fig:results_srl}
\end{figure}

==> explainability.tex <==
\chapter{Explainability on \kenn}\label{ch:expl}

==> implementation.tex <==
\section{Implementation}
\label{sec:implementation}

\TODO{Tagliare quasi tutto}

\kenn\ was developed as a python library built on top of TensorFlow 2.
% \TODO{tensorflow citation}


% \TODO{it is publicly available on \href{https://github.com/DanieleAlessandro/KENN}{github}.}

Such implementation makes an extensive usage of TensorFlow \emph{gather} and \emph{scatter\_nd} functions. Before entering the details about the class hierarchy of the library, lets introduce this two TensorFlow functions.

\section{tf.gather}
The \emph{gather} function of TensorFlow slices a given matrix according to an indices vector. Among the parameters of gather function there is the axis parameter, which determines if the matrix is sliced in rows or column vectors.

In Figure~\ref{fig:gather} an example of gather usage (with axis=0): given a matrix $X$ and an indices vector $i$, it returns a new matrix $Y$. The $j^{th}$ row of $Y$ is calculated as:
$$
Y_j = X_{i_j}
$$

Similarly, when the axis parameter is equal to 1, the resulting matrix $Y$ is obtaining by copying values from $X$ based on $i$. However, this time the slices are along the columns:
$$
Y^j = X^{i_j}
$$
where $Y^j$ is the $j^{th}$ column of $Y$.

For each value in $Y$, TensorFlow collects its original position on matrix $X$, meaning that it is capable of propagating back the error on matrix $X$ when calculating the gradients. In other words, gather is implemented as a differentiable operator.

\begin{figure}[H]
	\centering
	\input{tikz/gather_example}
    \caption{\emph{tf.gather} behaviour: given a matrix $X$ and an indices vector $i$, it copies in a new matrix the rows (columns) of $X$ based on the provided indices.}
    \label{fig:gather}
\end{figure}

For more details about \emph{tf.gather} please refer to the official \href{https://www.tensorflow.org/api_docs/python/tf/gather}{TensorFlow documentation}.

\section{tf.scatter\_nd}
Function \emph{tf.scatter\_nd} works in reverse of the \emph{gather} and, again, it is differentiable. With \emph{tf.gather}, the indices vector referred to the position of the inputs, this time they refers to the output matrix.

An example of the \emph{scatter} function (performed over the rows of $X$ and $Y$) in Figure~\ref{fig:scatter}.

If \emph{scatter\_nd} is performed over the rows, given a matrix $X$ and a indices vector $i$, the resulting matrix $Y$ is such that
$$Y_j = \sum_{k: \ i_k = j} X_k$$
where $k: \ i_k = j$ is the set of indices that satisfy the condition $i_k = j$. Similarly, when indices in $i$ corresponds to columns indices:
$$Y^j = \sum_{k: \ i_k = j} X^k$$

\begin{figure}[H]
	\centering
	\input{tikz/scatter_example}
    \caption{\emph{tf.scatter} behavior: it copies the rows (or columns) of a matrix in the position specified by the indices vector $i$. When multiple indices are equivalent it sums the corresponding rows (columns).}
    \label{fig:scatter}
\end{figure}

See \href{https://www.tensorflow.org/api_docs/python/tf/scatter_nd}{TensorFlow documentation} for more details about the \emph{scatter\_nd} function.

\section{The ClauseEnhancer class}

At the core of \kenn\ implementation there is the \emph{ClauseEnhancer} class, which extends keras Layer class.

A \emph{ClauseEnhancer} object is initialized by providing the list of all the predicates, a string representing the clause and the value of the default initial weight. Follows the signature of the \_\_init\_\_ method (constructor of the class) and its docstring:

\begin{python}
class ClauseEnhancer(tf.keras.layers.Layer):
    """Clause Enhancer layer

    """

    def __init__(self, available_predicates, clause_string, initial_weight_value):
        """Initialize the clause.

        :param available_predicates: the list of all possibleliterals in a clause
        
        :param clause_string: a string representing a conjunction of 
        literals. The format should be:
            clause_weight:clause
        
        The clause_weight should be either a real number (in such a case
        this sign is fixed) or an underscore (in this case the weight
        will be a tensorflow variable and learned during training).

        The clause must be represented as a list of literals separated by 
        commas (that represent disjunctions).
        
        Negation must specified by adding the letter 'n' before
        the predicate name.
        
        An example:
            _:nDog,Animal

        :param initial_weight_value: the initial sign to the clause 
        weight. Used if the clause weight is learned
        """
\end{python}


The \emph{ClauseEnhancer} class corresponds to a specific clause which is represented using three variables: \emph{gather\_literal\_indices}, \emph{scatter\_literal\_indices} and \emph{sign}. 

\emph{gather\_literal\_indices} corresponds to the indexes of the literals contained in the clause based on the order defined in the available\_predicates parameter of the \_\_init\_\_ method. It is a vector in $\Naturals^m$, where $m$ is the number of the clause's literals. For instance, if the list of predicates is $[Cat, Dog, Snake, Animal]$ and the clause is $\lnot Dog(x) \lor Animal(x)$, then $\emph{gather\_literal\_indices} = [1, 3]$. This variable is used by the \emph{gather} function to perform a $SELECT$ query.

\emph{scatter\_literal\_indices} is equivalent to the previous one, the only difference is the shape ($\Naturals^{m \times 1}$). The reason is that it is used by the \emph{scatter\_nd} function that requires as input a matrix instead of a vector.

Finally, \emph{sign} represents the sign of the literals. In the previous example: $\emph{sign} = [-1, 1]$ since the first literal $\lnot Dog(x)$ is negated while the second ($Animal(x)$) is not.

The key methods of Clause class are \emph{grounded\_clause} and \emph{call}. The \emph{grounded\_clause} method calculates the value of $\bz_c$ introduced in Section~\ref{sec:entire_knowledge}. Notice the usage of \emph{tf.gather} to select the pre-activations of the predicates involved in the clause and the multiplication for the \emph{self.sign} array to obtain the pre-activations of the literals.

\begin{python}
    def grounded_clause(self, inputs):
        """Find the grounding of the clause

        :param inputs: the tensor containing predicates' pre activations
        for many objects
        
        :return: the grounded clause (a tensor with literals truth values
        pre activations)
        """
        selected_predicates = tf.gather(inputs, self.gather_literal_indices, axis=1)
        clause_matrix = selected_predicates * self.signs

        return clause_matrix
\end{python}

The \emph{call} method returns the value of $\delta_c$ as described in Section~\ref{sec:entire_knowledge}. More in details, the usage of \emph{grounded\_clause} generates $\bz_c$ (denoted by \emph{clause\_matrix} in the code); the call of the TensorFlow \emph{softmax} function and the multiplication for \emph{self.clause\_weight} corresponds to the definition of $\delta^{w_c}_s$ (Equation~\ref{eq:delta_wc_s}); finally the multiplication for the \emph{self.sign} vector and application of \emph{scatter\_nd} calculates the value of $\delta_c$ as in Equation~\ref{eq:deltac}.

\begin{python}
    def call(self, inputs, **kwargs):
        """Improve the satisfaction level of the clause.
        
        :param inputs: the tensor containing predicates' pre-activation
        values for many entities
        :return: delta vector to be summed to the original pre-activation tensor
        to obtain an higher satisfaction of the clause"""
        clause_matrix = self.grounded_clause(inputs)

        delta = self.signs * tf.nn.softmax(clause_matrix) * self.clause_weight

        scattered_delta = tf.scatter_nd(self.scatter_literal_indices, \
         tf.transpose(delta), tf.reverse(tf.shape(inputs), [0]))

        return tf.transpose(scattered_delta)
\end{python}

\section{The knowledgeEnhancer class}
The \emph{knowledgeEnhancer} class is also an extension of the keras Layer class, and it is initialized with the same parameters as the ClauseEnhancer Class, except for the clause string which is substituted by a list of clause strings:

\begin{python}
def __init__(self, predicates, clauses, initial_clause_weight=0.5, **kwargs)
\end{python}

Indeed, the knowledge consists of a collection of clauses and for each of them, the knowledgeEnhancer internally builds a ClauseEnhancer. This is done by the build method of knowledgeEnhancer:

\begin{python}
def build(self, input_shape):
    for clause in self.clauses:
        self.clause_enhancers.append(ClauseEnhancer(self.predicates, \
                                                   clause[:-1], \
                                                   self.initial_clause_weight))

    super(KnowledgeEnhancer, self).build(input_shape)
\end{python}

The call method just need to apply each ClauseEnhancer to the input tensor and sum their results in roder to calculate the total change to be applied on the original pre-activations:

\begin{python}
def call(self, inputs, **kwargs):
    """Improve the satisfaction level of a set of clauses.

    :param inputs: the tensor containing predicates' pre-activation 
    values for many entities
    :return: final delta values"""

    deltas = []
    for clause in self.clause_enhancers:
        deltas.append(clause(inputs))

    return tf.add_n(deltas)
\end{python}

\section{The Kenn class}
All the previously defined keras layers are composed inside the Kenn class. This is the main class and it implements Equation~\ref{eq:final_intepretation}. A Kenn object can be seen as a wrapper for a \emph{KnowledgeEnhancer} object and its \emph{call} method just call the \emph{call} method of the \emph{KnowledgeEnhancer}, sums its results with the initial pre-activations tensor and applies the logistic function.

\begin{python}
    def call(self, inputs, **kwargs):
        """Improve the satisfaction level of a set of clauses.

        :param inputs: the tensor containing predicates' pre-activation values 
        for many entities
        :return: final preactivations"""

        deltas = self.knowledge_enhancer(inputs)

        return self.activation(inputs + deltas)
\end{python}

The Kenn class can not deal with relational data. This is the goal of the RelationalKenn class which uses two additional layers (the Join and GroupBy classes). Lets introduce them first.


\section{The Join class}
The Join class provides a call method which makes use of the gather function of TensorFlow to perform the JOIN query introduced in Section~\ref{sec:join}. It is implemented using the \emph{tf.gather} function. Differently from before, now the \emph{gather} function is applied over the rows of the matrix ($axis = 0$).

\begin{python}
def call(self, unary, binary, index1, index2):
    """Join the unary and binary tensors.

    :param unary: the tensor with unary predicates pre-activations
    :param binary: the tensor with binary predicates pre-activations
    :param index1: a vector containing the indices of the first object
    of the pair referred by binary tensor
    :param index1: a vector containing the indices of the second object
    of the pair referred by binary tensor
    """

    index1 = tf.squeeze(index1)
    index2 = tf.squeeze(index2)
    return tf.concat([tf.gather(unary, index1, axis=0),
                      tf.gather(unary, index2, axis=0),
                      binary], axis=1)

\end{python}

Here index1 and index2 are two vectors containing the indices of the two objects referred by matrix binary and they corresponds to the ``foreign keys'' of table binary (they are, respectively, $s^x$ and $s^y$ of Figure~\ref{fig:representation}).

\section{The GroupBy class}
Similarly to the Join class, GroupBy has a call method which performs the three queries introduced in Section~\ref{sec:groupby} (the SELECT query which returns $\delta \B$ and the two GROUP BY queries which calculate $\delta U_x$ and $\delta U_y$).

\begin{python}
    def call(self, unary, binary, deltas, index1, index2):
        """Split the deltas matrix in unary and binary deltas.

        :param unary: the tensor with unary predicates pre-activations
        :param binary: the tensor with binary predicates pre-activations
        :param deltas: the tensor containing the delta values
        :param index1: a vector containing the indices of the first object
        of the pair referred by binary and deltas tensors
        :param index1: a vector containing the indices of the second object
        of the pair referred by binary and deltas tensors
        """
        ux = deltas[:, :self.n_unary]
        uy = deltas[:, self.n_unary:2 * self.n_unary]
        b = deltas[:, 2 * self.n_unary:]
        shape = tf.shape(unary)

        return unary + tf.scatter_nd(index1, ux, shape) \
                     + tf.scatter_nd(index2, uy, shape),
               binary + b
\end{python}


\section{The RelationalKenn class}
The \emph{RelationalKenn} class implements the \kenn\ model introduced in Chapter~\ref{ch:architecture}. Its main purpose is to implement \kenn\ for the relational case. Although \emph{RelationalKenn} can be used also for knowledge bases composed uniquely by unary clauses, the efficiency is reduced since it makes use of Join and GroupBy layers and contains two different \emph{KnowledgeEnhancer} objects, one for the unary clauses and the other for binary clauses. For this reason, when the knowledge is composed only of unary clauses, Kenn class should be preferred.

The \emph{call} method performs the operations defined in Figure~\ref{fig:unary_binary}.

\begin{python}
def call(self, unary, binary, index1, index2, **kwargs):
    """Forward step of Kenn model for relational data.

    :param unary: the tensor with unary predicates pre-activations
    :param binary: the tensor with binary predicates pre-activations
    :param index1: a vector containing the indices of the first object
    of the pair referred by binary tensor
    :param index1: a vector containing the indices of the second object
    of the pair referred by binary tensor
    """

    if len(self.unary_clauses) != 0:
        u = unary + self.unary_ke(unary)
    else:
        u = unary

    if len(self.binary_clauses) != 0:
        joined_matrix = self.join(u, binary, index1, index2)
        deltas = self.binary_ke(joined_matrix)

        up, bp = self.group_by(u, binary, deltas, index1, index2)
    else:
        up = u
        bp = binary

    return self.activation(up), self.activation(bp)
\end{python}
 
\section{Parsers}
Parsers are functions that parse the knowledge bases files to generate the \emph{Kenn} and \emph{RelationalKenn} objects. The library contains two functions inside the parsers module: the \emph{unary\_parser} and the \emph{relational\_parser}. 

By decoupling the implementation of the model from the parsers of a specific type of knowledge files it is easier to extend the library to be used on different types of knowledge and different types of formats for the knowledge file.

\section{Usage}

\kenn\ library was developed with usability in mind. Indeed, in the simplest scenario only three lines of code are needed to inject the logic into a neural network model.
% \footnote{As previously mentioned, in the case of relational data one should also provide the two matrices with unary and binary predicates and the two indexes vectors}.

The following code is a simple example of a Multilayer Perceptron implemented useing keras:

\begin{python}
    import tensorflow as tf
    from tensorflow.keras.models import Sequential
    from tensorflow.keras.layers import Dense

    # Model definition
    model = keras.Sequential([
        Dense(100, activation="relu", name="layer1"),
        Dense(50, activation="relu", name="layer2"),
        Dense(5, activation="sigmoid", name="layer3")
        ])

    # Compile the model
    m.compile(
        optimizer='adam',
        loss='mean_squared_error')
\end{python}

\noindent Following, the previous code is changed to inject the knowledge:

\begin{python}
    import tensorflow as tf
    from tensorflow.keras.models import Sequential
    from tensorflow.keras.layers import Dense

    # **** 1 ****
    from kenn.parsers import unary_parser

    # Model definition
    model = keras.Sequential([
        Dense(100, activation="relu", name="layer1"),
        Dense(50, activation="relu", name="layer2"),
        # **** 2 ****
        Dense(5, activation="linear", name="layer3"),
        # **** 3 ****
        unary_parser('knowledge_file_path', activation=tf.nn.sigmoid)
        ])

    # Compile the model
    m.compile(
        optimizer='adam',
        loss='mean_squared_error')
\end{python}


\subsection{Example explained}
In the previous example, 3 changes have been applied to the original code. Following, the details.

\subsubsection{1. Import parser function}
The first change is trivial, we need to import the parser funtion from the library:

\begin{python}
    from kenn.parsers import unary_parser
\end{python}



\subsubsection{2. Change last layer activation}
Since \kenn\ works on the preactivations, the activation function of the last layer is changed from \emph{sigmoid} to \emph{linear}:

\begin{python}
    Dense(5, activation="linear", name="layer3")
\end{python}

\subsubsection{3. Inject the knowledge}
The parser function is used to read the file containing the knowledge and it returns the layer to be added on top of the base NN.

\begin{python}
    unary_parser('knowledge_file_path', activation=tf.nn.sigmoid)
\end{python}

\noindent Following, an example of knowledge base file:

\begin{verbatim}
    Dog,Cat,Animal,Car,Truck,Chair

    1.5:nDog,Animal
    _:nCat,Animal
    2.0:nDog,nCat
    _:nCar,Animal
    _:nAnimal,Dog,Cat    
\end{verbatim}}

\noindent The first row contains the list of predicates separated by commas and no spaces.
% Such a list defines the ordering of the predicates. When the KE is applied, it assumes that the columns of the input matrix contain the predicates ordered in the same way.
% \TODO{Each predicate must start with a capital letter. The second row must be empty. }
Other rows contain the clauses. Each clause is in a separate row and must be written respecting these properties:
\begin{itemize}
    \item logical disjunctions are represented with commas
    \item if a literal is negated, it must be preceded by the lowercase 'n'
    \item they must contain only predicates specified in the first row
    \item there shouldn't be spaces
\end{itemize}

Additionally, each clause must be preceded by a positive weight that represents the strength of the clause. More precisely, the weight could be a numeric value or an underscore: in the first case, the weight is fixed and determined by the specified value, in the second case the weight is learned during training.

For example, the third line represents the clause $\lnot Dog \lor Animal$. In this case, the clause weight is fixed to the value 1.5. 



% \TODO{dire qualcosa anche del caso relazionale}

% \TODO{Togliere qui sotto e [opz]spostarte in un altro capitolo}
% \section{Learning strategies}
% \begin{TODO LIST}{TODO}
% 	\item Entrare piu nel dettaglio delle differenze
% 	\item Aggiungere la possibilita di fissare i pesi
% 	\item Spostare?
% \end{TODO LIST}
% % \TODO{For all the experiments I used as NN a neural network with zero hidden layers, i.e., a logistic regression (LR).}
% Two learning strategies are possible: in the {\bfseries end-to-end} strategy, \kenn\ (base NN~+~KE) is trained end-to-end using the entire training set; with {\bfseries greedy} strategy the Training Set is splitted into two subset. With the first one the base NN is trained, with the second the KE (freezing the NN parameters). In the next chapters \kenn$_e$ and \kenn$_g$ will be used to distinguish between the two. 


% \TODO{TODO: spostare \\
% \kenn's hyper-parameters are the the same used for the base NN, with the addition of the initialization value for the clause weights.}



==> multilabel.tex <==

\section{Multi-label Classification with labels constraints}\label{sec:multilabel}

We need to evaluate two different aspects of \kenn: its ability to make use of the knowledge and the applicability of the model to relational domains. In this section we focus on the first aspect: the first experiments were conducted on three datasets for multilabel classification with no binary predicates. The next section will focus on evaluations on a relational domain.


\subsection{Multilabel classification tasks}
Multi-label classification is a supervised learning task relevant in many disciplines, e.g., bioinformatics~\citep{Yeast}, scene classification~\citep{multilabel_scene} and text categorization~\citep{text}. 

In multi-label classification we are interested in mapping specific observations to subsets of all the possible labels~\citep{multilabel,PF2008}.  It differs from binary classification and, more in general, from multi-class classification, because the classes are not mutually exclusive, i.e. multiple labels can be associated to a single instance. 

Formally, it is given a set of labels $\mathcal{L} = \left\{ \lambda_i | i=1...m \right\}$ and a training set $\mathcal{T} = \left\{ (x_i, y_i) | i=1...n \right\}$, where $x_i$ denotes features of the $i^{th}$ observation and the classification $y_i \in 2^{\mathcal{L}}$ is a subset of labels associated to such observation.  We want to find a classifier $\phi: \mathcal{X} \to 2^\mathcal{L}$ which, given features $x$ of an observation, returns the associated set of labels. 

\kenn\ is extremely suited to formulate multi-label classification with constraints. Indeed \kenn\ uses  vectorial representation for both features and corresponding classification, with $y_{i,j}$ equal to one if $\lambda_j$ is associated to observation $i$, zero otherwise.

While it is possible to train many different binary classifiers for each label, such a method does not take into account relationships among them. Indeed, in real-world applications, labels are often not independent. For this reason, it could be useful to exploit knowledge about labels relationships provided by some human experts. 

The prior knowledge $\clauses$ defined in~\ref{sec:prior_knowledge} represents the labels relationships that are represented in $\L$ as predicates.  For instance, a possible clause could be $\lambda_1 \lor \lnot \lambda_3 \lor \lambda_4$. Such a clause tells the system that at least one of the specified literal should be true.


% \TODO{
% More formally, it is given a prior knowledge $\clauses$ composed of a set of clauses. Each clause is a disjunction of (positive or negated) literals, each of which is a class (i.e., a label) of the multi-label classification problem. For instance, a possible clause could be $\lambda_1 \lor \lnot \lambda_3 \lor \lambda_4$. Such a clause tells the system that at least one of the specified literal should be true.}

% This first version of \kenn\ was limited and could not be used in the context of SRL. Notice that all the mentioned methods, except for KBANN, can deal with relational data and are suitable for solving SRL tasks. For this reason, I developed a new version of \kenn\ for which the aforementioned limitation is removed.}


We tested \kenn\ on three datasets: Yeast~\citep{Yeast_1}, Emotions~\citep{Emotions} and VRD Dataset~\citep{visual2}. Table~\ref{datasets} reports some figures of the three datasets. Please note that for VRD the features are two bounding boxes of an image together with the class of the contained object (there are 100 possible classes and we used as features the one-hot encoding of them plus the 4 coordinates of each bounding box).

	\begin{table}
		\caption{Datasets statistics}
		\centering
		\begin{tabular}{|l|l|l|l|l|}
			\hline
			Dataset & Features & Labels & Train & Test \\
			\hline
			\hline
			Yeast & 103 & 14 & 1500 & 917 \\
			\hline
			Emotions & 72 & 6 & 392 & 202 \\
			\hline
			VRD & 208 & 70 & 4000 & 1000 \\
			\hline
		\end{tabular}
		\label{datasets}
	\end{table}
	

\subsection{KENN with automatically generated knowledge}
\label{sec:yeast_emotions}
{
	
	
	\subsection{Yeast and Emotions datasets}
	Yeast dataset is a multilabel classification dataset for Bioinformatics. It contains 1500 training samples, each of which is composed of a vector of 103 features~\citep{Yeast_1, Yeast}. The features contain information about yeast microarray expressions. The 14 labels to be predicted are functional categories of yeast genes.
	
	The Emotions dataset contains features of songs of 7 types of different genres~\citep{Emotions}. Features were extracted from sounds clips of 30 seconds and they are divided into two categories: Rhythmic and Timbre. The labels are divided into 6 classes which represent different types of emotions.

	\subsection{Association rules learning for generating the knowledge}
	
	In our experiments on Yeast and Emotions datasets we used automatically extracted association rules. 
	
	Association rules learning is the task of extracting association rules from a database of transactions~\citep{rules_mining}. Given a set of items $\mathcal{I} = \mathcal{I}_1, \mathcal{I}_2 ... \mathcal{I}_n$, a transaction consists of an itemset $\mathcal{T} \subseteq \mathcal{I}$ and an association rule is an implication of the form ${\lambda_1 \land ... \land \lambda_n \to \lambda_j}$ that must hold in the dataset with a certain confidence.
	
	The idea is to use as prior knowledge for \kenn\ the association rules extracted from labels of the training set.
	
	For extracting association rules we used Apriori algorithm~\citep{Apriori}. As in~\citep{PF2008}, we generated each transaction from a sample using both positive and negative labels. More precisely, given a sample $(x_i, y_i)$, the transaction is calculated as:
	$$
	\Big\{ \lambda_j | y_{i,j} = 1 \Big\} \bigcup \Big\{ \lnot \lambda_j | y_{i,j} = 0 \Big\}
	$$
	where $\lambda_j$ is the $j^{th}$ label.
	
	\subsection{Experimental setup}
	In the experiments on both datasets, we used RMSProp~\citep{RMSProp} as learning algorithm.

	To select the best values for support and confidence of the Apriori algorithm we used a random search: we tried different combinations of values of the two hyperparameters to generate the rules. we used the generated rules to train \kenn\ using 2/3 of the Training Set and evaluated the model on the remain samples. Finally, the values that led to the highest accuracy were selected. Then, during the final evaluations, we used such optimal values for training \kenn\ using the entire Training Set.
	% for extracting rules from the entire Training Set and trained \kenn\ on it.

	Finally, we tried two learning strategies: in the \emph{end-to-end} strategy, we trained \kenn\ (base NN~+~KE) end-to-end using the entire training set; with \emph{greedy} strategy we split the training set into two subsets. With the first one we trained the base NN, with the second the KE (freezing the NN parameters). When showing results we will use \kenn$_e$ and \kenn$_g$ to distinguish between the two.

	It is worth noticing that, when using the greedy approach of learning, for every configuration tried for Apriori parameters the accuracy of \kenn\ was greater or equal than the one of the corresponding neural network, confirming the robustness of our method to poorly written knowledge bases.
	The found values for support and confidence are respectively 0.2 and 0.99 for Yeast Dataset and 0.2 and 0.7 for Emotions.




	% Among the hyper parameters there was also the initialization value for clause weights. The tried values ranged from 0 (the minimal possible value) to 10. It was clear pretty soon that high values greater than 2.0 performed much worse than smaller values. On the other hand, for small values there were no significant differences on the performances. I set the initial clause weight to 0.5. Such configurations was used also for later experiments, except when dealing with hard and reliable constraints (see Section~\ref{sec:VRD_settings} for more details).
	
	%An explanation can be that the number of clause weights is usually pretty small compared to the other parameters of the model and they are used only in the last layer: 

	% To select the best values of support and confidence for the Apriori algorithm we tried different combinations of values. We generated the rules and trained \kenn\ using 2/3 of the Training and evaluate the model on the remain samples. We finally kept the values with highest accuracy. Then we used the optimal value for extracting rules from the entire Training Set and trained \kenn\ on it.
	% It is worth noticing that, when using greedy approach of learning, for every configuration tried for Apriori parameters the accuracy of \kenn\ was greater or equal than the one of the corresponding neural network, confirming the robustness of our method to poorly written knowledge bases. The found values for support and confidence are respectively 0.2 and 0.99 for Yeast Dataset and 0.2 and 0.7 for Emotions.
	
	% In the same way I also tried to select the best initialization value for clause weight. There were no meaningful differences on the performances 

	\subsection{Results and discussion}
	% \begin{TODO LIST}{TODO}
	% 	\item ripetere esperimenti con un hidden layer (MLP)
	% 	\item Fare esperimenti con LTN (di nuovo, con LR e MLP)
	% 	\item Confronto
	% \end{TODO LIST}
	\label{sec:yeast_results}
	\begin{table}[t]
		\caption{Results with and without Prior Knowledge on Yeast and Emotions Datasets. The table shows Hamming Loss and Accuracy.}
		\centering
		\begin{tabular}{lllllll}
			&
			\multicolumn{1}{p{1.5cm}}{} &
			\multicolumn{2}{c}{Yeast} &
			\multicolumn{1}{p{0.5cm}}{} & \multicolumn{2}{c}{Emotions} \\
			\hline
			\rule{0pt}{3ex}
			& & HL & Acc & & HL & Acc \\
			\hline
			\rule{0pt}{3ex}\hspace{-0.12cm}
			& LR    & 22.38 & 37.52 &  & 27.89 & 33.70 \\
			& \kenn$_e$ & 22.24 & 46.43 & & 34.57 & 25.74 \\
			& \kenn$_g$   & \textbf{20.86}  & \textbf{48.56}  & & \textbf{24.59} & \textbf{38.78} \\
			\hline
			\hline
		\end{tabular}
		\label{YeastEmotions}
	\end{table}
	In Table~\ref{YeastEmotions} the final comparison between the logistic regression and \kenn: the usage of prior knowledge improved both HL and accuracy when using the greedy approach of learning, while the end-to-end one results in smaller improvements in Yeast dataset and a degradation in Emotions.
	
	In principle, we could expect better results training jointly the NN and KE,  because there could be some combinations of parameters for the entire model such that the NN performs poorly while the entire system gives good results.
	This type of configurations cannot be learned by the greedy approach. In other words, when training with the greedy approach, some solutions in the hypothesis space can not be reached.
	For this reason, the greedy approach has a smaller ability to fit the data. However, this could also imply an increased risk of overfitting.
	Therefore, we can expect better results of the end-to-end version when the amount of data is big enough to overcome overfitting.
	Indeed, the problem with the end-to-end version is visible in particular on the Emotions dataset, which has less than 400 samples for its training.



\subsection{Visual Relationship Detection}
\label{sec:VRD_experiments}
Visual Relationship Detection (VRD) is the task of finding objects in an image and capture their interactions~\citep{IvanThesis,visual2,visual1}. It is composed of three subtasks: Relationship Detection, Phrase Detection and Predicate Detection~\citep{visual2}. The general goal is to find relationships that are defined as triplets of the form $(subject, relation, object)$\footnote{in the original paper, the triplet was $(subject, predicate, object)$. Here we substituted $predicate$ with $relation$ to avoid ambiguity with the term ``predicate'' already in use}, where subject and object are defined with their class and a container bounding box. \DONE{Given an image, a bounding box of an object is the smallest rectangle that completely encloses the object and it is represented by the coordinates of the top left and the bottom right vertexes of the rectangle.}

An example of a relationship is the triplet $(person, kick, ball)$ in Fig.~\ref{fig:VRD}.

\kenn\ was evaluated only on the Predicate Detection task where subject and object are already given and the objective is to find only the relations. More in detail, in Predicate Detection two bounding boxes are given. The first one encloses the subject,  while the second contains the object. Together with the bounding boxes, the classes of the two contained objects are also given. The goal is to find the set of relations between the subject and the object.
Notice that each couple of objects can have multiple relations and the goal is to find all of them.

Moreover, even though the goal is to predict binary relations, we treated them as unary predicates by using the same strategy proposed in Section~\ref{sec:join}: a pair of bounding boxes is treated as a unique object and the binary predicates as unary predicates over the domain of pairs of bounding boxes. Notice that in this case we don't have to predict unary predicates in the original domain (the classes of the bounding boxes are already given) and for this reason, we don't need to use the RelationalKenn class.

\subsubsection{Visual Relationship Dataset}
% \TODO{Espandere... Guardando anche tesi di Ivan \\ }
% \TODO{altre immagini}
The Visual Relationship Dataset (VRD Dataset) is a dataset for Visual Relationship Detection. It contains 5000 images (4000 for training and 1000 for testing). Each image contains multiple objects, each of which is categorized based on its class. These classes include animals, vehicles, clothes, and other generic objects.

There are 100 classes that subject and object can take and 70 relations that have to be predicted which are divided into five types. Fig.~\ref{fig:VRD} shows the five types of relations in the VRD Dataset. The types are: Action (like Ride or Kick), Spatial (for example Below or On), Preposition (for example with or at), Comparative (like Taller) and Verb (for example Wear).

A triplet type is a triple $(subject class, relation class, object class)$ which corresponds to the classes of the two objects and the relation.

In total, the dataset contains 377993 relationship instances, with 6672 triplets types. Among the types of triplets, 1877 can be found only in the Test Set and predicting them is the goal of the Zero Shot Learning variant of the task. 


\begin{figure*}
    \makebox[\textwidth][c]{
        \includegraphics[scale=0.55]{Figures/VRD.png}
    }
    \caption{The five types of relations in VRD Dataset}
    \label{fig:VRD}
\end{figure*}

\subsubsection{The knowledge}
% \TODO{definire in modo formale i vari tipi di conoscenza (guardare anche paper PSL)}
We evaluated \kenn\ on the Predicate Detection task using the manually curated knowledge base described in \citep{IvanThesis}. This knowledge base contains 206 clauses divided in three groups:
% , namely:
\begin{description}
	\item[domain and range clauses] they restrict the domain (resp. range) of relations.
	\\Example of domain clause: $\lnot Wear(x,y) \lor Person(x)$ 
	\\Example of range clause: $\lnot ParkOn(x,y) \lor Street(y) \lor Road(y) \lor Grass(y)$
	\item[mutual exlusivity clauses] they represents mutual exsclusivity between to relations.\\
	An example is $\lnot Behind(x,y) \lor \lnot SitOn(x,y)$
	\item[sub-relation clauses] they state the containment between relations. An example:\\$\lnot Ride(x,y) \lor On(x,y)$)
\end{description}


\subsubsection{Experimental setup}
\label{sec:VRD_settings}
The experiments were carried out once again with Logistic Regression as Base NN. Notice that some of the clauses involve also unary predicates, which are given as input. For this reason, the architecture used is the one defined in Figure \ref{fig:KENN_inputs}, where the input predicates (classes of the bounding boxes) are concatenated with the predictions of the base NN before the application of the KE.

Although \kenn\ can learn clause weights, the presence of such parameters could slow down the learning process or cause overfitting. The system has to both use the knowledge and validate it. 
% \DONE{In contrast, LTN and SBR don't have this kind of problem, since in LTN there are no weights and in SBR the weights are provided as hyper parameters.}
Notice however that in \kenn\ clause weight can be added as constant values, in particular when the knowledge is reliable and the constraints are hard. For this reason, in VRD experiments, the domain and range clauses were treated as hard constraints: the clause weight was set to a high constant value (10.0) which was not learnable. This is because we know for sure that such rules are always satisfied.
% Moreover,each of them contains only one binary predicate (the other literals are all unary predicates already given as input).
% The other clause weights were initially set to 0.5 and then learned as described in Chapter~\ref{ch:kenn}. 

We trained both LR and \kenn\ using  RMSProp~\citep{RMSProp} and cross-entropy as the loss function. For evaluating the results we used the $Recall@n$ ($n \in \{50, 100\}$) metric proposed by Lu et al.~\citep{visual2} that is the percentage of times a correct relationship is found on the $n$ predictions with the highest score.


% \TODO{Espandere descrizione della metrica}

\subsubsection{Results and discussion}
\noindent Results on Predicate Detection task are shown in Table~\ref{table1}. 
\begin{table}[t]
	\centering
	\caption{Results on VRD Predicate Detection task \TODO{sistemare linea mezza bianca}}
	\begin{tabular}{llcclcc}
		&
		\multicolumn{1}{p{3.0cm}}{}
		& \multicolumn{2}{c}{Standard} &
		\multicolumn{1}{p{0.5cm}}{} &
		\multicolumn{2}{c}{Zero Shot} \\
		\hline
		\rule{0pt}{3ex}
		& & R@50           & R@100 & & R@50 & R@100 \\
		\hline
		& \rule{0pt}{3ex}\hspace{-0.12cm} \citep{visual2}  & 47.87          & 47.87 &    & 8.45            & 8.45 \\
	    & \citep{dai2017detecting} & 80.78 & 81.90 & &  - & - \\
		& \citep{Yu2017}  & 85.64          & \textbf{94.65} & & 54.20           & 74.65       \\
		& \citep{IvanThesis}        & 78.63          & 91.88   & & 46.28           & 70.15 \\
		& LR & 54.58 & 60.55 & & 33.88 & 44.91 \\
		& \kenn$_g$ & 59.87 & 71.42 & & 43.88 & 63.99 \\
		& \kenn$_e$       & \textbf{86.02} & 91.91 & &    \textbf{68.95}  & \textbf{83.83}  \\ 
		\hline
		\hline
	\end{tabular}
	\label{table1}
\end{table}
\kenn\ outperformed other methods on all the metrics except for Recall@100 of the standard variant of the task where it is surpassed by \citep{Yu2017}. Moreover, the best results of \kenn\  can be seen on Zero Shot Learning version where the difference between \kenn\ and the second best system is more than 10\%.
In \emph{Zero Shot Learning} the aim is to predict previously unseen triplets, therefore it is rather difficult to learn to predict them from the Training Set. This confirms the ability of \kenn\ to use the Knowledge Base. 

Another interesting result is the value obtained by \kenn\ compared to LTN~\citep{IvanThesis}. In particular considering that the two works used the same Prior Knowledge. A possible explanation is given by the ability of \kenn\ to learn \emph{clause weights}. Indeed, many weights results to be zero after learning. An example of a zero weighted clause is:~$\lnot Ride(x,y) \lor On(x,y)$.

Although the rule seems correct it is not in general satisfied in the training and test sets. This is because labels have been added manually, therefore there are plenty of missing relations. Our hypothesis is that people have a tendency to add the most informative labels making some of the clauses unsatisfied. For instance, suppose we need to label an image with a man riding a horse and we are not going to add all the relations since their number is pretty big (there are other objects and relations to label in the image, and multiple images). For the person and horse objects, there are plenty of different relations that are true: $Ride(x,y)$, $On(x,y)$, $Over(x,y)$, $Near(x,y)$ and so forth. It seems reasonable to think that a person that labels the image will tend to choose $Ride(x,y)$ over the others since it is the most informative one. This is because from $Ride(x,y)$ we can derive all the other relations. 
% \TODO{espandere, spiegare meglio, confrontare piu nel dettaglio con altri metodi, (collegare ad explainability?)}
%In other words, the clause $\lnot Ride(x,y) \lor On(x,y)$ is true, but it is exactly because it is true that it will be mostly false in the dataset.

Finally, notice that a perfect comparison between \kenn\ and LTN is difficult to obtain since the neural networks used in the two cases are different: \kenn\ is applied on a Logistic Regression network while LTN uses a Neural Tensor Network~\citep{NTN}. While it is possible to use the same NN in both cases, the NN architectures which works fine with one method do not work well with the other. See Section~\ref{sec:kenn_vs_sbr} for more details.

Another important aspect of the results is that \kenn\ increased the metrics values of LR. As in previous experiments on Yeast and Emotions (see Section~\ref{sec:yeast_emotions}), we tested \kenn\ both with greedy and end-to-end approaches. This time, although the greedy version brought improvements over the logistic regression, the best results are achieved by the end-to-end approach. This provides additional support for the overfitting hypothesis made in Section~\ref{sec:yeast_results} since VRD has a much bigger training set than Emotions and Yeast. Moreover, in previous experiments, prior knowledge was automatically extracted from the training data. Clauses could be satisfied within the training set just by chance. In such cases, the Apriori algorithm extracts misleading rules that are not satisfied at test time. This implies a further increase in the chances of overfitting.


% \subsection{Conclusions}\label{sec:conclusion4}
% With its results on the three analyzed datasets, \kenn\ showed to be able to efficiently exploit prior knowledge improving performances of the base neural network. Moreover, experiments on VRD dataset showed that \kenn\ is competitive against other approaches, in particular thanks to its ability to effectively learn \emph{clauses weights}.

% Finally, the evaluations analyzed in this chapter are focused on Multilabel classification tasks with no binary relations. In the next chapter we will presents the experiments on relational data and discuss the ability of \kenn\ to work in such contexts.

% despite \kenn\ performs better than LTN on Predicate Detection, it is restricted on multi-label classification tasks. This is because it requires preactivations to be stored in matrix $\bz$, which makes \kenn\ unable to work with general FOL clauses. In the next chapter we will discuss the extension of \kenn\ for relational data.

}


% \section{KENN with deep learning neural networks}
% {

% % \begin{quote}
% % \textit{One of the principal problem image forensics has to deal with is determining if a particular image is authentic or not. This task is very important in all those fields where is crucial to use such digital content as evidence like, for instance, in a court of law. To carry out such forensic analysis various technological instruments have been developed in literature. Many of them try to reveal if some modifications have been performed thus assessing that something of suspect could have been made, other ones search for comprehending what has happened and possibly which relations there are with other linked photos. In this chapter the problem of detecting if a feigned image has been created is investigated; in particular, attention has been paid to the case in which an area of an image is copied and then pasted onto another zone to make a duplication or to cancel something that was awkward.
% % To detect such modifications we propose a new methodology based on SIFT features. Our method allows both to understand if a copy-move attack has occurred and which are the image points involved, and, furthermore, to recover which has been the geometric transformation happened to perform cloning.
% % \footnote{A preliminary version of the work presented in this chapter has been published as \dquote{Geometric tampering estimation by means of a SIFT-based forensic analysis} in \textit{Proc.~of IEEE Int'l Conference on Acoustics, Speech, and Signal Processing (ICASSP), 2010},~\citep{ameriniICASSP} and submitted to IEEE Trans.~on Information Forensics and Security (TIFS).}
% % }
% % \end{quote}


% %-------------------------------------------------------------------------
% \subsection{Introduction}\label{sec:intro5}

% \begin{TODO LIST}{TODO}
%     \item Finora esperimenti solo con reti molto semplici
%     \item Dopo i risultati su Yeast ed Emotions con rete piu' grande di LR, diventa interessante capire se KENN puo' performare bene con rete deep
%     \item Abbiamo deciso di applicare KENN ad una CNN
%     \item Descrivere il problema del cibo e motivazioni
% \end{TODO LIST}

% %-------------------------------------------------------------------------
% \subsection{Food category dataset}\label{sec:food_category}
% \begin{itemize}
%     \item Descrivere il dataset (e link a github)
%     \item Descrivere il tipo di regole logiche
% \end{itemize}


% % \subsection{Our contribution}\label{sec:contribution5}


% %-------------------------------------------------------------------------
% % \section{The proposed method}\label{sec:three}



% % -------------------------------------------------------------------------
% \subsection{Experimental results}\label{sec:four}


% % -------------------------------------------------------------------------
% \subsection{Conclusion}\label{sec:five}

% }

% % \begin{quote}
% % \textit{In this chapter we introduce a novel multiple-logo matching and detection algorithm based on a new class of  similarity functions referred to as context dependent. Our approach is based on designing a similarity measure, involving interest points, which takes into account not only their intrinsic visual features but also their context and spatial configuration. The main contribution of this work includes (i) a variational framework which makes it possible to design our similarity as the fixed point of an energy function mixing a visual ``data term'', a ``context criterion'' and a ``regularization term'' and, (ii)  a theoretical study of the consistency of logo matching/detection and its invariance to different transformations including similarity and occlusion. Finally, we will show the validity of the method through extensive experiments on challenging logo images.  
% % \footnote{Part of this work was conducted while the author was a visiting Ph.D. student at XXXXX XXXXX, City (Nation), from Month to Month YEAR (working with. Dr.~Xxxx Yyyy). This chapter previously appeared as research report n.~2010D009, Xxxxx XXX~\citep{logocdk10}.}
% % }
% % \end{quote}


% %-------------------------------------------------------------------------
% \subsection{Introduction}\label{sec:intro4}
% TODO:
% \begin{itemize}
%     \item Esperimenti su VRD hanno mostrato che KENN funziona con una knowledge curata manualmente. Ci siamo chiesti se puo' funzionare anche con knowledge estratta automaticamente dal training set, come fatto in .... (citare articolo che usava regole logiche create da apriori)
%     \item Non e' detto: infatti le informazioni che stiamo aggiungendo sono ridondanti (gia' nel training set)
%     \item Abbiamo provato ad estrarre regole dalle labels del training set usando Apriori e testato se KENN aumentava le performances della rete base
% \end{itemize}

% %-------------------------------------------------------------------------
% \subsection{Yeast and Emotions datasets}\label{sec:intro4}
% Estendere di piu' rispetto all'articolo

% %-------------------------------------------------------------------------
% \subsection{Apriori algorithm}\label{sec:apriori}
% TODO: a partire da contenuto articolo PRICAI (espandere un po')

% %-------------------------------------------------------------------------
% \subsection{Methodology}\label{sec:methidology}
% TODO: spiegare settaggio rete e learning


% %-------------------------------------------------------------------------
% \subsection{Results}\label{sec:results}
% Dall'articolo

% %-------------------------------------------------------------------------
% \subsection{Discussion}\label{sec:discussion}
% TODO: sempre a partire dall'articolo
% Estendere:
% \begin{itemize}
%     \item Aggiungere risultati con rete con hidden layers
%     \item Aggiungere considerazioni su hypothesis space
%     \item Estendere discorso sulla differenza tra greedy e e2e
% \end{itemize}


% %-------------------------------------------------------------------------


% }

==> publications.tex <==
\chapter{Publications}
\label{app:publications}

\subsection*{Peer reviewed conference papers}
\begin{enumerate}
  \item \textbf{A. Daniele}, L. Serafini, ``Knowledge Enhanced Neural Networks'', \textit{PRICAI 2019: Trends in Artificial Intelligence}, pages: 542--554, 2019.\\
    \textbf{Candidate's contributions}: proposal of the initial idea, 
    theoretical analyses, development of the source code, evaluations.
  \end{enumerate}




==> tikz/z_histogram.tex <==
\newcounter{barcounter}

% A histogram chart with preactivations truth values and delta values
% Parameters:
%  #1          x position of the entire graph
%  #2          y position of the entire graph
%  #3          the name of the graph
\newenvironment{mygraph}[3]{
    \setcounter{barcounter}{0}

    \def\posx{#1}
    \def\posy{#2}

    \foreach \i in {0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,1.0}
    {
        \draw[ultra thin, fill=gray!0] (#1-0.1,#2+4*\i) -- (#1+6,#2+4*\i);
        \node[draw=none] at (#1-0.6,#2+4*\i) {\i};
    }
    




    % Draw one bar next to the previous one
    % Parameters:
    %  ##1          initial value
    %  ##2          label
    \newcommand{\mybar}[2]{
        \node[
            draw=none,
            fit={(#1+0.2+\value{barcounter}*1.2,#2) (#1+\value{barcounter}*1.2+1.2,#2+##1*4)},
            inner sep=0,
            outer sep=0,
            fill=gray!35] (#3B\arabic{barcounter}) {};

        \node[rotate=45,left] at (#1+\value{barcounter}*1.2+0.9,#2-0.1) {##2};

        \stepcounter{barcounter}
    }


    % Draw one bar next to the previous one with the green delta value
    % Parameters:
    %  ##1          initial value
    %  ##2          delta
    %  ##3          label
    \newcommand{\mybard}[3]{
        \node[draw=none,fit={(#1+0.2+\value{barcounter}*1.2,#2+##1*4) (#1+\value{barcounter}*1.2+1.2,#2+##1*4+##2*4)}, inner sep=0, outer sep=0, draw=none, fill=green!20] (#3D\arabic{barcounter}) {};

        \mybar{##1}{##3}

    }


    % Draw the last bar
    % Parameters:
    %  ##1          initial value
    %  ##2          label
    \newcommand{\mylastbar}[2]{
        \node[draw=none,fit={(#1+0.8+\value{barcounter}*1.2,#2) (#1+\value{barcounter}*1.2+1.8,#2+##1*4)}, inner sep=0, outer sep=0, draw=none, fill=gray!35] (#3Last) {};

        \node[rotate=45,left] at (#1+\value{barcounter}*1.2+1.4,#2-0.1) {##2};
    }

    % Draw the last bar with delta values
    % Parameters:
    %  ##1          initial value
    %  ##2          delta
    %  ##3          label
    \newcommand{\mylastbard}[3]{
        \node[draw=none,fit={(#1+0.8+\value{barcounter}*1.2,#2+##1*4) (#1+\value{barcounter}*1.2+1.8,#2+##1*4+##2*4)}, inner sep=0, outer sep=0, draw=none, fill=green!20] (#3LastD) {};

        \mylastbar{##1}{##3}
    }
}
{   
    \draw (\posx,\posy) -- (\posx+6,\posy);
    \draw[->] (\posx,\posy) -- (\posx,\posy+4.5);  
}
